Efficient numerical methods for the Maxey-Riley-Gatignol equations with Basset history term

The Maxey-Riley-Gatignol equations (MRGE) describe the motion of a finite-sized, spherical particle in a fluid. Because of wake effects, the force acting on a particle depends on its past trajectory. This is modelled by an integral term in the MRGE, also called Basset force, that makes its numerical solution challenging and memory intensive. A recent approach proposed by Prasath et al. exploits connections between the integral term and fractional derivatives to reformulate the MRGE as a time-dependent partial differential equation on a semi-infinite pseudo-space. They also propose a numerical algorithm based on polynomial expansions. This paper develops a numerical approach based on finite difference instead, by adopting techniques by Koleva et al. and Fazio et al. to cope with the issues of having an unbounded spatial domain. We compare convergence order and computational efficiency for particles of varying size and density of the polynomial expansion by Prasath et al., our finite difference schemes and a direct integrator for the MRGE based on multi-step methods proposed by Daitche. While all methods achieve their theoretical convergence order for neutrally buoyant particles with zero initial relative velocity, they suffer from various degrees of order reduction if the initial relative velocity is non-zero or the particle has a different density than the fluid.

==> appC.tex <==
% \label{appendix:c}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|| c | c | c | c | c | c ||} 
%    \hline
%    \multicolumn{6}{|c|}{Vortex flow field and zero initial relative velocity} \\
%    \hline
%    Method & $R=1/3$ & $R=7/9$ & $R=1$ & $R=4/3$ & $R=7/3$ \\ [0.5ex]
%    \hline\hline
%    Prasath et al. \cite{PrasathEtAl2019}& $2.07$ & $2.30$ & \textcolor{red}{machine-$\varepsilon$} & $2.46$ & $3.08$ \\
%    \hline
%    FD2 + Trap. & $2.00$ & $2.00$ & $2.02$ & $1.99$ & $1.99$ \\
%    \hline
%    FD2 + IMEX2 & $2.00$ & $2.00$ & $2.02$ & $2.00$ & $1.99$ \\
%    \hline
%    Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable} & $2.61$ & $3.13$ & $2.37$ & $2.39$ \\
%    \hline
%    FD4 + IMEX4 & $\textbf{3.21}$ & $\textbf{3.42}$ & $\textbf{4.01}$ & $\textbf{3.55}$ & $\textbf{3.66}$ \\
%    \hline
%    FD4 + DIRK4 & $\textbf{3.21}$ & $\textbf{3.42}$ & $3.39$ & $\textbf{3.55}$ & $\textbf{3.66}$ \\
%    \hline
% \end{tabular}
% \caption{Numerically computed convergence orders for paticles in the vortex for $S=0.1$ and different values of $R$. The initial conditions are $\bm{y}={(1,0)}^T$ and $\bm{q}(0,t_0)={(0,0)}^T$ and $t\in[0,1]$.}
% \label{table:convergence:vortex_R}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|| c | c | c | c | c | c | c ||}
%    \hline
%    \multicolumn{7}{|c|}{Vortex flow field and zero initial relative velocity} \\
%    \hline
%    Method & $S=0.01$ & $S=0.1$ & $S=0.5$ & $S=1$ & $S=2$ & $S=4$ \\ [0.5ex] 
%    \hline\hline
%    Prasath et al. \cite{PrasathEtAl2019} & $2.15$ & $2.46$ & $2.42$ & $3.41$ & $3.15$ & $\textbf{4.23}$ \\
%    \hline
%    FD2 + Trap. & $2.01$ & $1.99$ & $1.99$ & $1.99$ & $1.99$ & $1.98$ \\
%    \hline
%    FD2 + IMEX2 & $2.03$ & $2.00$ & $1.99$ & $1.99$ & $1.99$ & $1.99$ \\
%    \hline
%    Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable} & $2.37$ & $2.60$ & $2.67$ & $2.74$ & $2.79$ \\
%    \hline
%    FD4 + IMEX4 or DIRK 4& $\textbf{3.00}$ & $\textbf{3.55}$ & $\textbf{3.78}$ & $\textbf{3.84}$ & $\textbf{3.88}$ & $3.91$ \\
%    \hline
% \end{tabular}
% \caption{Numerically computed convergence orders for paticles in the vortex for $R=\nicefrac{4}{3}$ and different values of $S$. The initial conditions are $\bm{y}={(0,1)}^T$ and $\bm{q}(0,t_0)={(0,0)}^T$ and $t\in[0,1]$.}
% \label{table:convergence:vortex_S}
% \end{table}
% %
% %
% \begin{table}[h!]
% \centering
% \begin{tabular}{|| c | c | c | c | c | c ||} 
%    \hline
%    \multicolumn{6}{|c|}{Oscillatory background flow field and zero initial relative velocity} \\
%    \hline
%    Method & $R=1/3$ & $R=7/9$ & $R=1$ & $R=4/3$ & $R=7/3$ \\ 
%    \hline\hline
%    Prasath et al. \cite{PrasathEtAl2019} & $2.09$ & $2.30$ &  \textcolor{red}{machine-$\varepsilon$} & $2.44$ & $2.77$ \\
%    \hline
%    FD2 + Trap. & $1.97$ & $2.02$ & $2.02$ & $1.98$ & $1.97$ \\
%    \hline
%    FD2 + IMEX2 & $1.99$ & $1.98$ & $2.02$ & $1.98$ & $1.97$ \\
%    \hline
%    Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable} & $2.95$ & $3.08$ & $2.79$ & $2.78$ \\
%    \hline
%    FD4 + IMEX4 or DIRK4 & $\textbf{3.29}$ & $\textbf{3.51}$ & $\textbf{4.05}$ & $\textbf{3.64}$ & $\textbf{3.76}$ \\
%    \hline
% \end{tabular}
% \caption{Numerically computed convergence orders for the oscillatory background example with $S=0.1$ and different values of $R$. The initial conditions are $\bm{y}={(0,0)}^T$ and $\bm{q}(0,t_0)={(0,0)}^T$ and $t\in[0,1]$}
% \label{table:convergence:oscillatory_R}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|| c | c | c | c | c | c | c ||} 
%    \hline
%    \multicolumn{7}{|c|}{Oscillatory background flow field and zero initial relative velocity} \\
%    \hline
%    Method & $S=0.01$ & $S=0.1$ & $S=0.5$ & $S=1$ & $S=2$ & $S=4$ \\ [0.5ex] 
%    \hline\hline
%    Prasath et al. \cite{PrasathEtAl2019} & $2.15$ & $2.44$ & $2.49$ & $2.72$ & $2.51$ & $3.32$ \\
%    \hline
%    FD2 + Trap. & $2.02$ & $1.98$ & $1.96$ & $1.96$ & $1.96$ & $1.96$ \\
%    \hline
%    FD2 + IMEX2 & $1.98$ & $1.98$ & $1.97$ & $1.97$ & $1.97$ & $1.98$ \\
%    \hline
%    Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable} & $2.79$ & $2.84$ & $2.87$ & $2.89$ & $2.91$ \\
%    \hline
%    FD4 + IMEX4 or DIRK4 & $\textbf{3.01}$ & $\textbf{3.64}$ & $\textbf{3.76}$ & $\textbf{3.79}$ & $\textbf{3.79}$ & $\textbf{3.79}$ \\
%    \hline
% \end{tabular}
% \caption{Numerically computed convergence orders for a paticle in the the oscillatory background example with $R=\nicefrac{4}{3}$ and different values of $S$. The initial conditions are $\bm{y}={(0,0)}^T$ and $\bm{q}(0,t_0)={(0,0)}^T$ and $t\in[0,1]$}
% \label{table:convergence:oscillatory_S}
% \end{table}

% \begin{table}[h!]
%    \centering
%    \begin{tabular}{|| c | c | c | c | c | c ||} 
%        \hline
%        \multicolumn{6}{|c|}{Oscillatory background flow field and non-zero initial relative velocity} \\    
%        \hline
%        Method & $R=1/3$ & $R=7/9$ & $R=1$ & $R=4/3$ & $R=7/3$ \\ 
%        \hline\hline
%        Prasath et al. \cite{PrasathEtAl2019} & $\textbf{2.09}$ & $\textbf{2.30}$ & $\textbf{2.42}$ & $\textbf{2.43}$ & $\textbf{2.77}$ \\
%        \hline
%        FD2 + Trap. & $1.08$ & $1.00$ & $1.00$ & $1.01$ & $1.00$ \\
%        \hline
%        FD2 + IMEX2 & $1.11$ & $1.02$ & $1.01$ & $1.02$ & $1.01$ \\
%        \hline
%        Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable} & $1.77$ & $1.48$ & $1.55$ & $1.74$ \\
%        \hline
%        FD4 + IMEX4 or DIRK4 & $0.65$ & $0.64$ & $0.65$ & $0.67$ & $0.71$ \\
%        \hline
%    \end{tabular}
%    \caption{Numerically computed convergence orders for a particle in an oscillatory background with $S=0.1$ and different values of $R$. The initial conditions are $\bm{y}={(0,0)}^T$ and $\bm{q}(0,t_0)={(0,0.1)}^T$ and $t\in[0,1]$.}\label{table:convergence:oscillatory2_R}
% \end{table}

% \begin{table}[h!]
%    \centering
%    \begin{tabular}{|| c | c | c | c | c | c | c ||} 
%    \hline
%    \multicolumn{7}{|c|}{Oscillatory background flow field and non-zero initial relative velocity} \\    
%        \hline
%        Method & $S=0.01$ & $S=0.1$ & $S=0.5$ & $S=1$ & $S=2$ & $S=4$ \\ [0.5ex] 
%        \hline\hline
%        Prasath et al. \cite{PrasathEtAl2019} & $\textbf{2.15}$ & $\textbf{2.43}$ & $\textbf{2.48}$ & $\textbf{2.65}$ & $\textbf{2.56}$ & $\textbf{3.40}$ \\
%        \hline
%        FD2 + Trap. & $1.01$ & $1.01$ & $0.96$ & $0.94$ & $0.92$ & $0.91$ \\
%        \hline
%        FD2 + IMEX2 & $1.02$ & $1.02$ & $0.97$ & $0.95$ & $0.93$ & $0.92$ \\
%        \hline
%        Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable}& $1.55$ & $1.61$ & $1.67$ & $1.76$ & $1.87$ \\
%        \hline
%        FD4 + IMEX4 or DIRK4 & $0.64$ & $0.67$ & $0.68$ & $0.68$ & $0.68$ & $0.68$ \\
%        \hline
%    \end{tabular}
%    \caption{Numerically computed convergence orders for a paticle in a oscillatory background with $R=\nicefrac{4}{3}$ and different values of $S$. The initial conditions are $\bm{y}={(0,0)}^T$ and $\bm{q}(0,t_0)={(0,0.1)}^T$ and $t\in[0,1]$.}\label{table:convergence:oscillatory2_S}
% \end{table}


% \begin{table}[h!]
%    \centering
%    \begin{tabular}{|| c | c | c | c | c | c ||} 
%        \hline
%        \multicolumn{6}{|c|}{Quiescent flow field and non-zero initial relative velocity} \\    
%        \hline
%        Method & $R=1/3$ & $R=7/9$ & $R=1$ & $R=4/3$ & $R=7/3$ \\ 
%        \hline\hline
%        Prasath et al. \cite{PrasathEtAl2019} & $\textbf{1.71}$ & $\textbf{2.22}$ & $\textbf{2.45}$ & $\textbf{2.71}$ & $\textbf{3.86}$ \\
%        \hline
%        FD2 + Trap. or IMEX2 & $1.00$ & $1.00$ & $1.00$ & $1.00$ & $1.00$ \\
%        \hline
%        Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable} & $1.82$ & $1.35$ & $1.37$ & $1.39$ \\
%        \hline
%        FD4 + IMEX4 or DIRK4 & $0.65$ & $0.65$ & $0.65$ & $0.66$ & $0.66$ \\
%        \hline
%    \end{tabular}
%    \caption{Numerically computed convergence orders for a particle in a quiescent flow with $S=0.1$ and different values of $R$. The initial conditions are $\bm{y}={(0,0)}^T$ and $\bm{q}(0,t_0)={(0.1,0)}^T$ and $t\in[0,1]$.}
%    \label{table:convergence:quiescent_R}
% \end{table}

% \begin{table}[h!]
%    \centering
%    \begin{tabular}{|| c | c | c | c | c | c | c ||} 
%        \hline
%        \multicolumn{7}{|c|}{Quiescent flow field and non-zero initial relative velocity} \\        
%        \hline
%        Method & $S=0.01$ & $S=0.1$ & $S=0.5$ & $S=1$ & $S=2$ & $S=4$ \\ [0.5ex] 
%        \hline\hline
%        Prasath et al. \cite{PrasathEtAl2019} & $\textbf{1.95}$ & $\textbf{2.71}$ & $\textbf{3.14}$ & $\textbf{3.74}$ & $\textbf{3.35}$ & $\textbf{4.84}$ \\
%        \hline
%        FD2 + Trap. or IMEX2 & $1.00$ & $1.00$ & $0.99$ & $0.98$ & $0.97$ & $0.96$ \\
%        \hline
%        Daitche $3^{rd}$ order \cite{Daitche2013} & \textcolor{red}{unstable} & $1.37$ & $1.24$ & $1.24$ & $1.27$ & $1.30$ \\
%        \hline
%        FD4 + IMEX4 or DIRK4& $0.64$ & $0.66$ & $0.67$ & $0.68$ & $0.68$ & $0.68$ \\
%        \hline
%    \end{tabular}
%    \caption{Numerically computed convergence orders for a paticle in a quiescent flow with $R=\nicefrac{4}{3}$ and different values of $S$. The initial conditions are $\bm{y}={(0,0)}^T$ and $\bm{q}(0,t_0)={(0.1,0)}^T$ and $t\in[0,1]$}
%    \label{table:convergence:quiescent_S}
% \end{table}
